Stealing Machine Learning Models via Prediction APIs

Machine learning (ML) models may be deemed confidential due to their sensitive training data, commercial value, or use in security applications. Increasingly often, confidential ML models are being deployed with publicly accessible query interfaces. ML-as-a-service ("predictive analytics") systems are an example: Some allow users to train models on potentially sensitive data and charge others for access on a pay-per-query basis. The tension between model confidentiality and public access motivates our investigation of model extraction attacks. In such attacks, an adversary with black-box access, but no prior knowledge of an ML model's parameters or training data, aims to duplicate the functionality of (i.e., "steal") the model. Unlike in classical learning theory settings, ML-as-a-service offerings may accept partial feature vectors as inputs and include confidence values with predictions. Given these practices, we show simple, efficient attacks that extract target ML models with near-perfect fidelity for popular model classes including logistic regression, neural networks, and decision trees. We demonstrate these attacks against the online services of BigML and Amazon Machine Learning. We further show that the natural countermeasure of omitting confidence values from model outputs still admits potentially harmful model extraction attacks. Our results highlight the need for careful ML model deployment and new model extraction countermeasures.

==> amazon.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Dealing with Unknown Model Classes or Hyperparameters} 
\label{sec:amazon}

\tnote{Update this. We will add some results on improper extraction as well as
our reverse engineering forays}

In modern services such as Amazon's ML and Google's Prediction API, the details
of training algorithms are not made public. In other contexts APIs allow users to tune 
hyper-parameters, meaning they will not necessarily be known to an attacker that
later gets access to a trained model's prediction functionality. Both situations
can be modeled in our formalism above by having $\trainalg$ select from the
various options randomly according to some distribution (e.g., uniformly).
In this section we describe several strategies that can assist one in
determining these unknowns.

\paragraph{Model type shattering proofs.} Consider a situation in which 
an adversary does not know what model class is being used by a service, but has
the ability to train and use models on the service. A mechanism to
rule out certain model types is based on the well known theory of VC
dimension~\cite{vapnik-etal}. Fix some class of models $\modelclass$. 
For
example, this could be all models that are linear functions. A model $f
\in \modelclass$ is said to shatter a set of  
$s$ points  $\xvec_1,\ldots,\xvec_s \in \fspace$ if $f$ ... 

shattering set
for a model class $\modelclass$ is a set of $s$ points in $\fspace$ such that
...\tnote{fix this. It's not clear VC dimension is the right intuition for what
we want to do with a dimensionality witness. By the latter I mean one or more 
training sets for which no classifier from a model class can achieve 100\%
accuracy on the training set.}

To rule out model types with VC dimension less than $d$, then, first generate a
training set that is a $d$-shattering set. Train a model using this set, and
then determine the error of the resulting model on the training set. Should the
service use a model class with VC dimension less than $d$ there will
\emph{necessarily} be non-zero error. Repeating this for several values
values of $d$ (perhaps using binary search) will identify the minimal $d$ for
which the service can train a fully accurate classifier.

\paragraph{The extract-and-test approach.}  Consider a setting in which one
knows a set of extraction strategies $\advA_1,\ldots,\advA_k$ 
achieving functionally equivalent success rates $\epsilon_1,\ldots,\epsilon_k$
when the target model uses a 


\paragraph{Case study: Amazon Machine Learning.} The Amazon service allows users
to upload training sets, request a model be trained from these training sets,
and then obtain predictions using the resultant model. Users can control some
aspects of the training process, but not all: a specification of the feature
space $\fspace$; a specification of the range $\range$ and whether one is
performing classification or regression;  options for feature normalization
and binning\tnote{fill in details}; the training set itself; and 
permissions on whom can perform prediction queries against the resulting model. 
The information in the documentation suggests that we ...\tnote{fill in some
details about what we can infer from it about the remainder of the reverse
engineering tasks discussed below. For example, that we should turn off certain
binning features or whatever.}

Notably absent from documentation is a description of the actual training
procedure $\trainalgAmazon$ used. Comments on online forums suggest the use of
logistic and multinomial regression.  We therefore use this as a case study in
the difficulty of narrowing in on the exact model class and hyperparameters of an 
unknown ML service. We apply the two techniques discussed above.

\emph{Dimension witnesses.} We carefully crafted a synthetic dataset
that forms a non-linearity witness. This can be as small as four data points,
with labels such that there exists no linear classifier able to achieve 100\%
accuracy on training data. We then trained a model on Amazon using this data;
the full set of options are given in the appendix.\fixme{fill in appendix if we
think this is interesting enough} Using the prediction API we measure the
error on the training set, and the resulting 100\% accuracy reveals
non-linearity. Note that this rules out the use of conventional logistic or
multinomial regression. \tnote{Should we add diagram? Fan's circle-in-circle
picture is pretty good, though maybe simpler witnesses shoudl be shown} 

\anote{It's not clear that there is a \emph{universal} set of points that proves a particular VC dimension $d$. Fan's example applies to a particular model class---linear models. This is something to look into. A model class has VC dimension $d$ if there exists a set of $d$ points that it shatters. So there may not exist a compact ``positive'' dimensionality witness, i.e., a set of inputs that proves VC dimension at least $d$. And it may not be possible to construct a size-$d$ ``negative'' dimensionality witness that proves that the VC dimension is less than $d$, as there must exist no such set for the VC dimension to be less than $d$.}


%user-controlled options for training appear in \figref{fig:amazon-api}.

\emph{Extract-and-test approach.} \tnote{fix this wording} The ability to classify highly non-linear
arrangements of points, combined with the hypothesized use of logistic
regression, suggests the use of kernel techniques. Kernelized logistic
regression (KLR), as described in \secref{sec:background}, picks a subset of
training points to serve as representers and then applies some kernel function
with these points when performing classification.

%\begin{figure}[t]
%\center\footnotesize
%\begin{tabular}{|l|l|}
%\hline
%Option & Description \\
%\caption{Amazon ML user-customizable options.}
%\label{fig:amazon=-api}
%\end{figure}

\paragraph{Case study 2: Logistic regression in BigML}


==> data/regression/bin/preamble.tex <==
%--------------
%% preamble.tex
%% this should be included with a command like
%% \input{preamble.tex}
%% \lecture{1}{September 19, 2012 }{Aleksander Madry}{name of poor scribe}
% % Template based on Dan Spielman's template

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[theorem]{Assumption}

%\newcommand{\qed}{\rule{7pt}{7pt}}
\newcommand{\dis}{\mathop{\mbox{\rm d}}\nolimits}
\newcommand{\per}{\mathop{\mbox{\rm per}}\nolimits}
\newcommand{\area}{\mathop{\mbox{\rm area}}\nolimits}
\newcommand{\cw}{\mathop{\rm cw}\nolimits}
\newcommand{\ccw}{\mathop{\rm ccw}\nolimits}
\newcommand{\DIST}{\mathop{\mbox{\rm DIST}}\nolimits}
\newcommand{\OP}{\mathop{\mbox{\it OP}}\nolimits}
\newcommand{\OPprime}{\mathop{\mbox{\it OP}^{\,\prime}}\nolimits}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\abs}[1]{\left| #1 \right|}

%\newenvironment{proof}{\noindent{\bf Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-sketch}{\noindent{\bf Sketch of Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-of-lemma}[1]{\noindent{\bf Proof of Lemma #1}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-attempt}{\noindent{\bf Proof Attempt}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proofof}[1]{\noindent{\bf Proof}
of #1:\hspace*{1em}}{\qed\bigskip}
\newenvironment{remark}{\noindent{\bf Remark}\hspace*{1em}}{\bigskip}

%\newcommand{\FOR}{{\bf for}}
%\newcommand{\TO}{{\bf to}}
%\newcommand{\DO}{{\bf do}}
%\newcommand{\WHILE}{{\bf while}}
%\newcommand{\AND}{{\bf and}}
%\newcommand{\IF}{{\bf if}}
%\newcommand{\THEN}{{\bf then}}
%\newcommand{\ELSE}{{\bf else}}

\newcommand{\ord}{{\rm ord}}

\providecommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\embed}{{\rm Embed}}
\newcommand{\qembed}{\mbox{$q$-Embed}}
\newcommand{\calh}{{\cal H}}
\newcommand{\lp}{{\rm LP}}

\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Ints}{\mathbb{Z}}

\newcommand*\rot{\rotatebox{90}}
\newcommand*\OK{\ding{51}}
\newcommand*\NOK{\ding{55}}


\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\set}[1]{\left\{ #1 \right\}}



\newcommand{\fvec}{\mathbf{f}}
\newcommand{\xvec}{\mathbf{x}}
\newcommand{\yvec}{\mathbf{y}}
\newcommand{\wvec}{\mathbf{w}}
\newcommand{\betavec}{\boldsymbol{\beta}}
\newcommand{\alphavec}{\boldsymbol{\alpha}}
\newcommand{\fspace}{\mathcal{X}}
\newcommand{\ispace}{\mathcal{M}}
\newcommand{\msg}{M}
\newcommand{\fdim}{d}
\newcommand{\range}{\mathcal{Y}}
\newcommand{\tree}{T}
\newcommand{\id}{\texttt{id}}
\newcommand{\oracle}{\mathcal{O}}
\newcommand{\ext}{\textsf{ex}}



\newcommand{\naSucc}{\textnormal{p-Succ}}
\newcommand{\Succ}{\textnormal{Succ}}
\newcommand{\AttSucc}{\textnormal{AttSucc}}
\newcommand{\TRAINACC}{\textnormal{ACC}}
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}

\newcommand{\algorithmiccontinue}{\textbf{continue}}
\newcommand{\Continue}{\State \algorithmiccontinue}
\newcommand{\True}{\texttt{True}}
\newcommand{\False}{\texttt{False}}





\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}{c@{\hspace*{.5em}}c}
        \begin{minipage}{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.2}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.2}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.2}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.2}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.2}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.2}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.2}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.2}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.2}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\apref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
%\newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}


\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}


\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}




\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}


\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{0pt}$\bullet$\hfill}{\labelwidth=10pt%
\labelsep=0pt \leftmargin=10pt \topsep=1pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=0pt \leftmargin=22pt \topsep=1pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt} }}{\end{list}}

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\pgfplotscreateplotcyclelist{list}{%
{color=red,solid,mark=x},
{color=blue,dashed,every mark/.append style={solid},mark=diamond},
{color=teal,dotted,every mark/.append style={solid},mark=square},
{color=brown,dashdotted,every mark/.append style={solid},mark=o},
{color=black,dashdotdotted,every mark/.append style={solid},mark=triangle},
{color=orange,solid,every mark/.append style={solid},mark=*}}

\pgfplotsset{
  every axis plot/.append style={line width=0.8pt},
  every axis plot post/.append style={
    every mark/.append style={line width=0.8pt}
  }
}

\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, black, align=center, inner sep=2pt,
                     top color=white, bottom color=blue!20},
  inner/.style      = {treenode, thin},
  leaf/.style    = {circle,black, thin, draw,inner sep=0.5pt},
  leafShade/.style    = {circle,OliveGreen,thick,draw,inner sep=0.5pt, text=black}
}


% Complex \xxx for making notes of things to do.  Use \xxx{...} for general
% notes, and \xxx[who]{...} if you want to blame someone in particular.
% Puts text in brackets and in bold font, and normally adds a marginpar
% with the text ``xxx'' so that it is easy to find.  On the other hand, if
% the comment is in a minipage, figure, or caption, the xxx goes in the text,
% because marginpars are not possible in these situations.
{\makeatletter
 \gdef\xxxmark{%
   \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
     \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
       \marginpar{\textcolor{red}{xxx~}}% not in a caption or minipage, can use marginpar
     \else
       \textcolor{red}{xxx~}% notice trailing space
     \fi
   \else
     \textcolor{red}{xxx~}% notice trailing space
   \fi}
 \gdef\xxx{\@ifnextchar[\xxx@lab\xxx@nolab}
 \long\gdef\xxx@lab[#1]#2{{\bf [\xxxmark \textcolor{red}{#2} ---{\sc #1}]}}
 \long\gdef\xxx@nolab#1{{\bf [\xxxmark \textcolor{red}{#1}]}}
}


\def\authnotes{1}

\newcounter{notectr}[section]
\newcommand{\thenote}{\thesubsection.\arabic{notectr}\refstepcounter{notectr}}

\newcommand{\note}[2]{$\ll$#1~\thenote: #2$\gg$}
\newcommand{\tnote}[1]{\ifnum\authnotes=1 \textcolor{blue}{\note{TomR}{#1}}\fi}
\newcommand{\tcrnote}[1]{\tnote{#1}}
\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\anote}[1]{\ifnum\authnotes=1 \textcolor{red}{\note{AJ}{#1}}\fi}
\newcommand{\fnote}[1]{\ifnum\authnotes=1 \textcolor{brown}{\note{FT}{#1}}\fi}
\newcommand{\znote}[1]{\ifnum\authnotes=1 \textcolor{purple}{\note{Fan}{#1}}\fi}




\newcommand{\inspace}{\mathcal{I}}
\newcommand{\outspace}{\mathcal{Y}}
\newcommand{\classes}{\mathcal{C}}
\newcommand{\hypclass}{\mathbb{H}}
\newcommand{\numclasses}{c}
\newcommand{\thh}{^\textrm{th}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\fout}{\hat{f}}
\newcommand{\featext}{\phi}
\newcommand{\kernel}{K}
\newcommand{\kernelrbf}{\kernel_{\mathrm{rbf}}}
\newcommand{\kernelquad}{\kernel_{\mathrm{quad}}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\cdotsm}{\cdot\hspace*{-2pt}}


\newcommand{\splitfun}{\rho}

\newcommand{\trainalg}{\mathcal{T}}
\newcommand{\trainHide}{\mathcal{H}_\trainalg}
\newcommand{\trainalgAmazon}{\mathcal{T}_{\textrm{amazon}}}

\newcommand{\rangedist}{d}

\newcommand{\setting}{\textsf{S}}
\newcommand{\testset}{D}
\newcommand{\unifset}{U}
\newcommand{\distclass}{\mathcal{P}}
\newcommand{\error}{R}
\newcommand{\errortest}{\error_{\mathrm{test}}}
\newcommand{\errortesttv}{\error_{\mathrm{test}}^{\mathrm{TV}}}
\newcommand{\errorunif}{\error_{\mathrm{unif}}}
\newcommand{\erroruniftv}{\error_{\mathrm{unif}}^{\mathrm{TV}}}
%\newcommand{\loss}{L}
%\newcommand{\avgloss}{\overline{L}}
%\newcommand{\losstest}{L_\mathrm{test}}
%\newcommand{\losstestreal}{L_\mathrm{test}}
%\newcommand{\lossunif}{L_{\mathrm{unif}}}
%\newcommand{\lossexact}{L_{\mathrm{sd}}}
%\newcommand{\lossatt}{L_\mathrm{app}}
%\newcommand{\avglosstest}{\overline{L}_\mathrm{test}}
%\newcommand{\losstestreal}{L_\mathrm{test}}
%\newcommand{\avglossunif}{\overline{L}_{\mathrm{unif}}}
%\newcommand{\avglossexact}{\overline{L}_{\mathrm{sd}}}
\newcommand{\traindist}{p}
\newcommand{\testdist}{q}
\newcommand{\extractdist}{r}
\newcommand{\naEXTGAME}{\textnormal{P-MLEXT}}
\newcommand{\EXTGAME}{\textnormal{MLEXT}}

\newcommand{\modelclass}{\mathcal{C}}

\newcommand{\getdisttrain}{{\;\leftarrow_{\traindist}\;}}
\newcommand{\getdisttest}{{\;\leftarrow_{\testdist}\;}}
\newcommand{\getsr}{{\;{\leftarrow{\hspace*{-2pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\;}}

\newcommand{\advA}{\mathcal{A}}
\newcommand{\advB}{\mathcal{B}}


\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\Probb}[2]{\Pr[#1]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

\newcommand*\rotcol{\rotatebox{90}}

\newcommand{\ie}{{i.e.,~}}
\newcommand{\eg}{{e.g.,~}}



==> evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

We evaluated the efficiency of our model extraction attacks on a large range of models, trained over both synthetic and real datasets. For efficiency reasons, we run most of our evaluations locally, using either public APIs provided by ML services or models trained locally using state-of-the-art learning algorithms. However, we do also show-case examples of online attacks against real ML services. We note that while some of our adaptive attacks (i.e. those for decision trees) may require each query to be sent individually to an API, others can benefit from \emph{batch predictions}, that are supported by all major MLaaS platforms we reviewed.

\subsection{Experimental Setup}

With the notable exception of decision trees, the model classes introduced in \secref{sec:prelims} follow a precise mathematical formulation, and we thus expect various ML services to define these models in equivalent ways. Although the training procedures themselves may be subject to more variation (such as data splitting or the choice of hyper-parameters), we can still assume that they rely on one of a few popular state-of-the art optimization techniques. For SVMs and logistic regressions, we make use of the implementations available in the popular \texttt{scikit} library. As we describe in \secref{sec:amazon}, we find that, unsurprisingly, our local implementation produces the same outputs as the BigML API, for the binary and OvR logistic regressions that it supports. 

For kernelized regression and neural nets, we build a local learning algorithm based on the \texttt{theano} optimization library. We use standard accelerated stochastic gradient descent to solve the optimization problems encountered during training and extraction of a model. We train multi-layer perceptrons with a single hidden layer of $3$ to $20$ hidden nodes, with the $\tanh$ activation function. When training logistic regressions with an RBF kernel, we randomly select a fixed number of training samples as representers, and choose the value of $\gamma$ through cross-validation. For both training and extraction, we run at most $1000$ epochs of $1000$ batches each.

The decision tree model presented in \secref{sec:prelims} matches that used by BigML, and incorporates the most common type of splits found in other implementations. For our experiments, we downloaded a number of publicly available decision tree models from BigML (see Figure~\ref{fig:benchmark-trees}), and query them locally using available BigML API bindings. We first generated a small number of online queries to models with restricted black-box access, to discover what information is contained in the service's responses. We then simulate black-box oracle access locally, by discarding any extra information returned by the API on a membership query.

\paragraph{Datasets}

\paragraph{Query Budget \& Success Rate}

For each extracted model $f'$, we evaluate the losses $\losstest$ and $\lossunif$ with respect to the true model $f$. We approximate $\losstest$ as the mis-classification rate over the full collected datasets, and $\lossunif$ as the mis-classification rate over a set sampled uniformly from $\fspace$. For decision trees, $\fspace$ is reported by the BigML API (even for black-box models), and we sample each feature uniformly in its range. For other models, we uniformly sample from $\fspace = [-1, 1]^\fdim$. For models that produce class probabilities, we also evaluate $\losstest$ and $\lossunif$ using the total-variation distance between $f(\xvec)$ and $f'(\xvec)$.

For our decision tree extraction algorithms, the number of performed membership queries depends only on the initial query $\xvec_{init}$ and on the target granularity $\epsilon$ for continuous features. We evaluate the average success and query budget of our attacks by repeating the attacks for multiple randomly chosen initial queries (note that the top-down strategy always starts with an initially empty query, and is thus fully deterministic for a choice of $\epsilon$).

For the other model types, our extraction strategies can be parametrized by a query budget $m$. We evaluate our attacks' success for increasing query budgets, by varying $m$ as a factor of the total number of \emph{unknown parameters} $k$ that comprise the oracle model $f$ (this is precisely the number of unknowns in the optimization problems or equation systems that we solve in our extraction attacks). For each trained model, we run each strategy with query budgets $\alpha \cdot k$, for $0.5 \leq \alpha \leq 100$, and record the attack's success rate. \fnote{Should we also record extraction time?}


\subsection{Results}
\label{sec:results}

\paragraph{Linear Models}

%\begin{figure*}[t]
%   \centering
%   \include[width=\textwidth]{data/regression/bin/full_plot}
%   \caption{Average loss of extracted linear models for different extraction strategies.}
%   \label{fig:results:linear}%
%\end{figure*}

We evaluate the Lowd \& Meek attack, our $3$ retraining strategies, and the equation solving attack given class probabilities, for binary logistic regression models trained over the binary datasets in Figure~\ref{fig:benchmark}.
These models have $d+1$ parameters, and we vary the budget as $\alpha \cdot (d+1)$ for each dataset.
We plot the average losses $\avglosstest$ and $\avglossunif$ over all linear models, as a function of $\alpha$ in Figure~\ref{fig:results:linear}.

As we can see, the retraining strategies that search for points near the decision boundary perform better than simply retraining over uniform samples. However, the Lowd \& Meek approach of directly solving for the unknown parameters $\wvec$ and $\beta$ is much more accurate that finding these parameters through log-loss minimization. When class probabilities are available, $d+1$ uniform queries are sufficient to solve the obtained linear system to arbitrary precision.

As we noted in \secref{sec:linear}, none of the strategies that rely only on class labels can guarantee that the extracted parameters will be close to the true ones, because the decision boundary is invariant under scaling. in Figure~\ref{fig:results:linear}, we show this by comparing the class probabilities predicted by the different extracted models.

\paragraph{Multiclass Logistic Regression}
\fnote{Will add these later. The results are essentially similar to the binary case, except that Lowd \& Meek doesnt apply here.}

\paragraph{Neural Nets}

%\begin{figure*}[t]
%\footnotesize
%   \centering
%   \include[width=\textwidth]{data/nnets/full_plot}
%   \caption{Average loss of extracted neural nets for different extraction strategies.}
%   \label{fig:results:nnets}%
%\end{figure*}

\paragraph{SVM with RBF kernel}

\paragraph{Decision Trees}

\paragraph{Extracting Training Data from Kernel Models}


==> linear.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Extraction Strategies}
\label{sec:strategies}

For our extraction attacks, we assume that the adversary gets black-box oracle access to some model $f$, from one of the \emph{model classes} $\hypclass$ introduced in Section~\ref{sec:prelims}. For simplicity, we further assume that the adversary knows the particular model class to which $f$ belongs, along with its potential hyper-parameters. We note that in popular ML services, this information is often publicly available or it can be inferred from available documentation and interaction with the model. We discuss inference of model classes and hyper-parameters in more detail in Section~\ref{sec:amazon}. We first focus on general extraction strategies for oracle models that only output class labels, and no class probabilities.

A particularity of this setting is that, as in PAC learning~\cite{PAC}, for any set of queries $\xvec_i \in \fspace$ and corresponding oracle responses $y_i \in \outspace$, there actually is a model $f'$ in $\hypclass$ (namely $f$), for which $f'(\xvec_i) = y_i, \forall i$. This assumption on the target function has been criticized as unrealistic in the PAC learning framework, which has notably lead to the relaxed notion of agnostic learning~\cite{agnostic}. However, for the model extraction attacks we consider, this assumption is indeed reasonable since the oracle $f$ we wish to extract is not some arbitrary, naturally occurring function, but rather a particular type of machine learning model trained by a specific ML service.

This suggests a simple `retraining approach' to model extraction: obtain a number of samples $(\xvec_i, y_i) \in \fspace \times \outspace$ from the oracle $f$, and find a model $f'$ that produces the same classifications as $f$ for those samples. The PAC learning literature has produced concrete upper-bounds on the generalization error for such retraining approaches, for many classes of models~\cite{PAC}. These do not directly apply here however for two reasons. First, we do not assume that the adversary knows the target distribution $\traindist$ (specifically its marginal distribution on $\fspace$), implying that the queried samples do not necessarily come from $\traindist$. Rather, we consider adversaries that make either uniform queries or arbitrary membership queries to the oracle.
Secondly, we care about average case rather than worst-case success of our extraction strategies, for those classes of models that are typically encountered in ML services. We thus resort to empirical evaluation of our attacks' success, for a number of real-world models.\\

We introduce three classes of extraction strategies, that broadly apply to all model classes introduced in Section~\ref{sec:prelims}, except for decision trees. We discuss extraction attacks on decision trees in more detail in Section~\ref{sec:dectrees}. The main difficulty of tree models, compared to the other model classes we consider, is in actually finding a model $f'$ than produces the same classifications as $f$, given only black-box oracle access. The following three classes of retraining strategies issue $m$ queries to the oracle, and receive back class labels.

\begin{enumerate}
\item \textbf{Retraining with uniform queries.} This baseline strategy simply consists in sampling $m$ points $\xvec_i \in \fspace$ uniformly at random, querying the oracle, and training a model $f'$ on these samples.
\item \textbf{Active retraining with membership queries.} This strategy applies techniques from active learning~\cite{active}. For some round number $r$, it first queries the oracle on $\frac{m}{r}$ uniform points, and trains a model $f'$. It then selects $\frac{m}{r}$ new points, along the decision boundary of $f'$ (these are intuitively the points $f'$ is least \emph{certain} about), and sends those to the oracle. This iterative improvement of the model $f'$ is repeated $r$ times, at which point $m$ membership queries have been issued.
\item \textbf{Online retraining with membership queries.} This strategy consists of adaptively issuing $m$ membership queries to the oracle, to find samples close to the decision boundaries of $f$ (using line search techniques). A model $f'$ is then trained on the $m$ queried samples.
\end{enumerate}

In Sections~\ref{sec:linear}-\ref{sec:dectrees}, we discuss how these strategies may be instantiated for particular model classes. We will also introduce more specific extraction attacks that only apply to certain model classes, and may assume richer output from the oracle (such as class probabilities).



\subsection{Linear Models}
\label{sec:linear}

\paragraph{Lowd \& Meek's attack}
In~\cite{LowdMeek}, Lowd and Meek present a simple attack on any linear classifier, assuming black-box oracle access with membership queries. A linear classifier is defined by a weight vector $\wvec \in \R^\fdim$ and a threshold $\beta \in \R$, and classifies an instance $\xvec$ as \emph{positive} if $\wvec \cdot \xvec + \beta > 0$ and \emph{negative} otherwise. SVMs with linear kernels and binary logistic regressions are examples of linear classifiers. Their attack consists in using line searches to find points arbitrarily close to the decision boundary of $f$ (points for which $\wvec \cdot \xvec + \beta \approx 0$), and reconstruct $\wvec$ and $\beta$ (up to some arbitrary scaling factor) from these samples.

\paragraph{Linear SVMs}
Given a training set of $n$ points of the form $((\xvec_1, y_1), \cdots,
(\xvec_n, y_n))$, a linear SVM is the ``maximum-margin hyperplane'', defined by the equation $\wvec \cdot \xvec + \beta = 0$, 
that separates the points $x_i$ for which $y_i=1$ from the points for which $y_i = 0$.

The most obvious extraction strategy is to simply retrain a SVM on samples obtained from the oracle $f$, using one of the three aforementioned retraining strategies. Since the samples returned by $f$ must be linearly separable, the retraining strategies will converge to a model $f'$ that linearly separates these samples as well, and hopefully approximates the true hyperplane well.

Naturally, $f$'s  hyperplane can also be determined by finding points
arbitrarily near the decision boundary and directly solving the system of
equations of unknowns $\wvec$ and $b$ (similarly to Lowd \& Meek). If the oracle
$f$ outputs auxiliary information, such as the distance from the decision
boundary to the point being queried, the hyperplane can be determined by solving
a system of equations, as the (signed) distance from $\xvec$ to the hyperplane
defined as above is $\frac{\wvec \cdot \xvec + \beta} {\|\wvec\|}$.

\paragraph{Binary Logistic Regression}

Logistic regression models are typically trained by minimizing the \emph{cross-entropy loss} (also called \emph{logistic loss}). This loss approximates the ideal $0$-$1$ loss by strongly penalizing misclassified samples. Specifically, given $m$ samples $(\xvec, y_i)$ from $f$, where $y_i \in \set{0,1}$, we search the model $f'$ (with parameters $\wvec', \beta')$ that minimizes $\sum_{i=1}^m\sum_{j=0}^{1} \mathbbm{1}_{\set{y_i = j}} \cdot \log(f'_{j}(\xvec_i))$. If a regularization term $\lambda \cdot \norm{\wvec'}_2^2$, where $\lambda > 0$, is added to the loss function, the optimization problem is \emph{strongly convex}, implying that a global minimum can be found efficiently. As the samples $(\xvec_i, y_i)$ obtained from $f$ are linearly separable, setting $\lambda$ to a sufficiently low positive value guarantees that we will find an $f'$ that linearly separates the samples as well.

If the oracle $f$ provides class probabilities, extraction of a binary logistic regression simply reduces to solving a linear system of equations. Indeed, we have that $\wvec \cdot \xvec + \beta = \sigma\left(\frac{f_1(\xvec)}{1-f_1(\xvec)}\right)$. Thus, querying the oracle with $\fdim$ linearly independent queries $\xvec$ suffices to extract a model $f'$ that is identical (up to numerical precision) to $f$. Note that the Lowd \& Meek attack does not have such strong guarantees, as it extracts coefficients $\wvec'$, $\beta'$ that may be scaled from $\wvec$, $\beta$ by some arbitrary positive factor. 






==> neural.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Non-Linear Models}
\label{sec:nonlinear}

Lowd \& Meek's attack on linear classifiers does not extend to multi-class models with (multiple) linear decision boundaries or to models with non-linear decision boundaries. The same line search techniques can be used to find points near a decision boundary of $f$, but extracting the actual model $f$ from these points is more difficult. We thus resort to the $3$ retraining strategies introduced previously. As for binary logistic regression models, we will see that the availability of class probabilities rather than class labels only leads to much more efficient extraction models.

\paragraph{Multiclass Regression}

The extraction attacks for softmax regression are essentially generalizations of those for binary logistic regression. Training a softmax regression with $c>2$ classes also entails minimizing the cross-entropy loss, given by $\sum_{i=1}^m\sum_{j=0}^{c} \mathbbm{1}_{\set{y_i = c}} \cdot \log(f'_{j}(\xvec_i))$, for $m$ oracle samples $(\xvec_i, y_i)$. Again, this optimization problem can be made strongly convex by the addition of a regularization term, implying that an optimal solution (that correctly classifies all $m$ samples) can be found using traditional optimization techniques.

If class probabilities are available, $\wvec$ and $\beta$ can be extracted by solving a non-linear system of equations (one sample $(\xvec, y)$ gives rise to $c$ equations of the form $[f_0(\xvec), \dots, f_{c-1}(\xvec)] = y$). Such a system can be efficiently solved through the same optimization procedure used to train the regression in the presence of class labels only, by minimizing the cross entropy $\sum_{i=1}^m\sum_{j=0}^{c} f_j(\xvec_i) \cdot \log(f'_j(\xvec_i))$. Note however, that unlike in the binary case, there is no guarantee that we recover $\wvec$ and $\beta$ exactly, because the softmax function is \emph{shift-invariant} (i.e. applying a constant linear shift to all $\wvec_i$ or all $\beta_i$ does not change the outputs of $f$). We may thus succeed in extracting a model $f'$ that is \emph{functionally equivalent} to $f$ (i.e $f(\xvec) = f'(\xvec)\; \forall \xvec \in \fspace$), yet $f$ and $f'$ may not have the same parameters. \\

The case of one-vs-rest (OvR) regression is more delicate. Indeed, in this case $f$ consists of $c$ binary models that jointly define a decision boundary that separates each class from the rest. However, this does not imply that each of the $c$ classes can be linearly separated from \emph{all} the others. Thus, if the oracle only responds to sample queries with class labels, the different retraining strategies might not succeed in extracting a model $f'$ that agrees with $f$ on those samples. We will evidence this particularity in our experimental results in Section~\ref{sec:eval}, and comment on its implications on potential countermeasures to model extraction in Section~\ref{sec:countermeasures}.

If the oracle provides class probabilities however, we can use the same approach as for softmax regression and directly extract the \emph{combination} of $f$'s $c$ binary models, by solving a non-linear system of equations in the parameters $\wvec$ and $\beta$. For this, we can not re-use any existing implementations of OvR regression (since these solve $c$ separate optimization problems), but can make use of any state-of-the-art non-linear system solver. As far as we know, OvR regression does not have any scale- or shift-invariance property, implying that we may succeed in extracting $\wvec$ and $\beta$ exactly, up to the precision of the optimization procedure.

\paragraph{Neural Networks}
The multilayer perceptrons we consider, are essentially generalizations of softmax regression with an additional hidden layer. The main difference is that the cross-entropy loss function for neural nets is not strongly convex, even if regularization terms are added. For instance, note that any re-ordering of the hidden layers and corresponding weights does not change the function $f$. Thus, the minimization problems we consider (either over class labels or class probabilities) have multiple local optima, and depending on the network architecture and transfer function used, there is no guarantee that we will find a global minima of the cross entropy loss. As we will see in Section~\ref{sec:eval}, we do nevertheless succeed in extracting models with low $\losstest$ and $\lossunif$ in practice, especially when class probabilities are provided.


\paragraph{SVMs with non-linear Kernels}

Here we consider two commonly used kernels, namely the polynomial kernel and RBF kernel. Extracting an SVM with polynomial kernel can be reduced to extracting a linear SVM in the transformed feature space. Indeed, a projection function $\phi(\cdot)$ can be derived from any given polynomial kernel function so that $K_{\text{poly}}(\xvec, \xvec')=(\xvec^T\cdot \xvec' + 1)^d$ can be written as $K_{\text{poly}}(\xvec, \xvec')=\phi(\xvec)^T \cdot \phi(\xvec')$. This actually transforms the kernelized SVM into a linear one, since the decision function now becomes $f(\xvec)=\text{sign}(\phi(\xvec) \cdot \wvec^{F} + \beta)$ where $\wvec^F= \sum_{i=1}^t \alpha_i \phi(\xvec_i$. We can employ techniques from Section \ref{sec:linear} to efficiently extract $\wvec^F$ and $\beta$ as long as $\phi(\xvec)$ is feasible to compute.

However this nice property of polynomial kernels does not apply to RBF kernels since the projection function for an RBF kernel produces an infinite-dimensional vector. Here we instead resort again to the retraining idea.  Training a kernelized SVM (in dual form) is to find the $\alpha_i$ that maximize $\sum_i \alpha_i - \frac{1}{2}\sum_i \sum_j y_i \alpha_i y_j \alpha_j K(\xvec_i, \xvec_j)$ subject to $0 \le \alpha_i \le \frac{1}{2n\lambda}$ and $\sum_i \alpha_i y_i = 0$. Just as for linear models, mis-classification is strongly penalized by setting $\lambda$ to a small positive value. 
%Nonetheless, unlike in the case of linear models, there is no guarantee that the $f'$ obtained by the retraining procedure is exactly the $f$. But empirically, as we show in the experiment section, $\lossunif$ and $\losstest$ converge to zero quickly with reasonably amount of retraining samples.

\paragraph{Logistic Regression with RBF Kernel}

The above discussions on extractions of softmax regressions and SVMs with RBF kernels directly extend to kernelized logistic models. However, as we will demonstrate in our evaluations, an interesting (yet dangerous) particularity of these models is that an attacker may succeed in extracting not only a close approximation of $f$, but also actual samples from the model's training data. Indeed, the model parameters of $f$ consist not only of learned weights $\alphavec$ and $\betavec$, but also of a random subset of the training data (used as representers for the RBF kernel). If $f$ outputs class probabilities, each sample $(\xvec, y)$ defines $c$ equations over the unknown weights and representer vectors of $f$. This assumes that the adversary knows the number $s$ of representers used in the model. However, note that `augmenting' $f$ with additional representers with corresponding weights $\alpha = 0$ does not change $f$'s output. Thus, even if the adversary over-estimates the number of representers used in $f$, he may still construct a system of equations whose optimal solution is a model equivalent to $f$, and thus potentially succeed in extracting training data. Furthermore, as we show in our experiments, leakage of training data may even occur if the adversary severely under-estimates the actual number of representers in $f$.


